Neighborhood Convolutional Network: A New Paradigm of Graph Neural Networks for Node Classification

The decoupled Graph Convolutional Network (GCN), a recent development of GCN that decouples the neighborhood aggregation and feature transformation in each convolutional layer, has shown promising performance for graph representation learning. Existing decoupled GCNs first utilize a simple neural network (e.g., MLP) to learn the hidden features of the nodes, then propagate the learned features on the graph with fixed steps to aggregate the information of multi-hop neighborhoods. Despite effectiveness, the aggregation operation, which requires the whole adjacency matrix as the input, is involved in the model training, causing high training cost that hinders its potential on larger graphs. On the other hand, due to the independence of node attributes as the input, the neural networks used in decoupled GCNs are very simple, and advanced techniques cannot be applied to the modeling. To this end, we further liberate the aggregation operation from the decoupled GCN and propose a new paradigm of GCN, termed Neighborhood Convolutional Network (NCN), that utilizes the neighborhood aggregation result as the input, followed by a special convolutional neural network tailored for extracting expressive node representations from the aggregation input. In this way, the model could inherit the merit of decoupled GCN for aggregating neighborhood information, at the same time, develop much more powerful feature learning modules. A training strategy called mask training is incorporated to further boost the model performance. Extensive results demonstrate the effectiveness of our model for the node classification task on diverse homophilic graphs and heterophilic graphs.

==> 3Analysis.tex <==
% In this section, we first provide the complexity analysis of \name. 
% Then we discuss the connections between \name and decoupled GCN, which is the last 

% \subsection{Complexity Analysis}
% We analyze the time complexity and space complexity of \name as follows.

% \textit{Time complexity.} 
% The time complexity of \name depends on two parts, i.e., convolutional layers and fully-connection layers. Their time complexities are $O(nd^{\prime}K^2)$ and $O(ndd^{\prime}+ nd^{\prime}c)$, respectively, where $n$ is the number of nodes, $K$ is the propagation step, $c$ is the number of labels, $d$ and $d^{\prime}$ denote the dimension of the raw feature vector and the hidden feature vector, respectively. Thus, the total complexity of \name is $O(nd^{\prime}K^2 + ndd^{\prime}+ nd^{\prime}c)$. Since the values of $K$ and $c$ are always very small, the time complexity can be $O(ndd^{\prime})$. Comparing to decoupled GCN which has $O(mKc + ndc)$ given that $m$ is the number of edges, \name is more efficient to perform on the dense graphs in which the number of edges is much larger than the number of nodes. It is because the time complexity of decoupled GCN relies on both $n$ and $m$, while the time complexity of \name depends on only $n$.

% \textit{Space complexity.}
% The space complexity of \name depends on two parts, i.e., model parameters and intermediate variables. 
% Their space complexities are $O(K+dd^{\prime}+d^{\prime}c)$ and $O(bKd^{\prime})$, respectively,
% and the total space complexity of \name is $O(bKd^{\prime}+dd^{\prime}+d^{\prime}c)$, where $b$ denotes the batch size.
% Comparing to decoupled GCN which has $O(nc + dc + m)$, \name is more scalable on large-scale graphs as the space cost of \name does not count the size of graph.


















% In this section, we theoretically illustrate that decoupled GCN can be replaced by a two-steps method which first aggregates the neighborhood features via the propagation operation and then extracts the representation of nodes using CNN. Furthermore, we discuss the limitations of decoupled GCN based on the theoretical analysis.

% We first prove that the representation of nodes learned by decoupled GCN can be also extracted by using CNN based on the information of multi-hop neighborhoods. We have the lemma as follows.

% \textbf{LEMMA 1.} \textit{For any node $v_i$, the representation of node $v_i$ learned by decoupled GCN with $K$ steps could be also extracted by performing a convolutional layer with kernel size $K$, given as $[\alpha_0,\cdots,\alpha_K]^{\top}\in \mathbb{R}^{(K+1)\times 1}$, on the multi-hop neighborhood features.}

% %Here $K$ denotes the total propagation step, and $\alpha_0,\cdots,\alpha_K$ are the aggregation weights of decoupled GCN.

% \begin{proof}
% According to \autoref{eq:dgcn}, for any node $v_i$, the representation feature $\mathbf{Z}_{i} \in \mathbb{R} ^ {1 \times d^{\prime}}$ can be caluculated as $\mathbf{Z}_{i} = \sum_{k=0}^{K} \alpha_{k} \mathbf{H}_{i}^{(k)}$, 
% where $\mathbf{H}_{i}^{(k)}\in \mathbb{R} ^ {1 \times d^{\prime}}$ denotes the feature of the $k$-hop neighborhood aggregated by a propagation method.

% On the other hand, \autoref{eq:dgcn} can be regarded as a two-steps process, namely calculating the feature for each hop of neighborhood and aggregating the features of all hops. For the first step, the calculated features of multi-hop neighborhoods of node $v_i$ can be given as $\{\mathbf{H}_{i}^{(0)},\cdots,\mathbf{H}_{i}^{(K)}\}$. Then, we can generate a grid-like feature matrix $\mathbf{T}_{i}\in \mathbb{R} ^ {(K+1) \times d^{\prime}}$ by stacking the calculated features, such that

% % : first calculating the features of multi-hop neighborhoods and then utilizing the aggregating weights $\alpha_0,\cdots,\alpha_K$ to aggregate the features from multi-hop neighborhoods.
% % For the first step, we can obtain the features of multi-hop neighborhoods of node $v_i$ as $\{\mathbf{H}_{i}^{(0)},\cdots,\mathbf{H}_{i}^{(K)}\}$.
% % We further stack them according to the ascending order of propagation steps, generating a grid-like feature matrix $\mathbf{T}_{i}\in \mathbb{R} ^ {(K+1) \times d^{\prime}}$:
% \begin{equation}
%   \mathbf{T}_{i}=[\mathbf{H}_{i}^{(0)},\cdots,\mathbf{H}_{i}^{(K)}]^{\top}= \begin{bmatrix}
% 	\mathbf{H}_{i,0}^{(0)} & \mathbf{H}_{i,1}^{(0)} & \cdots & \mathbf{H}_{i,d^{\prime}}^{(0)} \\
% 	\mathbf{H}_{i,0}^{(1)} & \mathbf{H}_{i,1}^{(1)} & \cdots & \mathbf{H}_{i,d^{\prime}}^{(1)} \\
% 	\vdots&\vdots& \ddots&\vdots\\
% 	\mathbf{H}_{i,0}^{(K)} & \mathbf{H}_{i,1}^{(K)} & \cdots & \mathbf{H}_{i,d^{\prime}}^{(K)} \\
% 	\end{bmatrix}.
% 	\label{eq:grid-f}
% \end{equation}
% Thus, aggregating the features with weights $\alpha_0,\cdots,\alpha_K$ can be regarded as a convolutional layer\footnote{For simplicity, the items of bias are ignored.} in which the convolutional kernel is $[\alpha_0,\cdots,\alpha_K]^{\top}\in \mathbb{R}^{(K+1)\times 1}$.

% Finally, we can obtain the representation $\mathbf{Z}^{\prime}_{i}\in \mathbb{R} ^ {1 \times d^{\prime}}$ by conducting the convolutional layer on the grid-like feature matrix $\mathbf{T}_{i}$, such that
% % By performing such a convolutional layer on the grid-like feature matrix $\mathbf{T}_{i}$ of node $v_i$, we can obtain the output representation $\mathbf{Z}^{\prime}_{i}\in \mathbb{R} ^ {1 \times d^{\prime}}$:
% \begin{equation}
% \begin{aligned}
%   \mathbf{Z}^{\prime}_{i} & = [\mathbf{H}_{i}^{(0)},\cdots,\mathbf{H}_{i}^{(K)}]^{\top} \oplus
%   [\alpha_0,\cdots,\alpha_K]^{\top}\\
%     & = \sum_{k=0}^{K} \alpha_{k} \mathbf{H}_{i}^{(k)} = \mathbf{Z}_{i},
% 	\label{eq:con-gf}
% \end{aligned}   
% \end{equation}
% where $\oplus$ denotes the convolution operation.
% \end{proof}

% According to \textbf{LEMMA 1}, we can find that the calculation process of decoupled GCN can be considered as performing a  convolution operation on the grid-like feature matrix. However, there are two main limitations of decoupled GCN as follows. On the one hand, it is hard to capture the informative representations for the features of nearby hops. Since decoupled GCN utilizes only a single convolutional layer which covers the whole grid-like feature matrix, the convolutional kernel can not extract the local representations for the features of nearby hops. For example,

% On the other hand, the impact of the original features of nodes are underestimated. As discussed, decoupled GCN leverages a convolutional layer to generate the node representation from its multi-hop neighborhoods.
% The attribute feature of the node itself, an essential part of the node characteristics, is overlooked since the convolutional layer is developed to extract the features of multi-hop neighborhoods.  
% The lack of the attribute feature of the node itself could lead to learning the suboptimal node representation, further hurting the model performance for the downstream tasks.

% % preserve the local association information of each feature


% % Since decoupled GCN utilizes a single convolutional layer to extract the features of multi-hop neighborhoods, the selection of the convolution kernel is crucial.
% % And the kernel size of decoupled GCN is $(K+1)\times 1$, which aims to capture the high-level semantic information of each feature among all neighborhoods. 
% % Intuitively, The association between adjacent neighborhoods is more potent than that of nonadjacent neighborhoods. 
% % However, such a large receptive field can not preserve the local association information of each feature in multi-hop neighborhoods well,
% % causing it hard to capture the meaningful information of multi-hop neighborhoods.

% % decoupled GCN first transforms the information of multi-hop neighborhoods of a node into a grid-like feature matrix and perform once convolution operation via a single convolutional layer with fixed kernel size on the grid-like feature matrix to generate the node representation.
% % Such a working mechanism could suffer from two limitations:
% % \begin{enumerate}
% % \item \textit{Hard to capture the informative features from the complex information of multi-hop neighborhoods.} 
% % Since decoupled GCN utilizes a single convolutional layer to extract the features of multi-hop neighborhoods, the selection of the convolution kernel is crucial.
% % And the kernel size of decoupled GCN is $(K+1)\times 1$, which aims to capture the high-level semantic information of each feature among all neighborhoods. 
% % Intuitively, The association between adjacent neighborhoods is more potent than that of nonadjacent neighborhoods. 
% % However, such a large receptive field can not preserve the local association information of each feature in multi-hop neighborhoods well,
% % causing it hard to capture the meaningful information of multi-hop neighborhoods.

% % \item \textit{Overlooking the features of nodes themselves.}
% % As discussed, decoupled GCN leverages a convolutional layer to generate the node representation from its multi-hop neighborhoods.
% % The attribute feature of the node itself, an essential part of the node characteristics, is overlooked since the convolutional layer is developed to extract the features of multi-hop neighborhoods.  
% % The lack of the attribute feature of the node itself could lead to learning the suboptimal node representation, further hurting the model performance for the downstream tasks.
% % \end{enumerate}

% % To address the above limitations, we proposed a more general and powerful framework called \textbf{N}eighborhood \textbf{C}onvolutional \textbf{N}etwork (\name).
% % We detail the design of \name in the next Section.

